Locally adaptive estimation methods with application to univariate time series

The paper offers a unified approach to the study of three locally adaptive estimation methods in the context of univariate time series from both theoretical and empirical points of view. A general procedure for the computation of critical values is given. The underlying model encompasses all distributions from the exponential family providing for great flexibility. The procedures are applied to simulated and real financial data distributed according to the Gaussian, volatility, Poisson, exponential and Bernoulli models. Numerical results exhibit a very reasonable performance of the methods.

==> conclusion.tex <==
\section*{Conclusion}
\label{sec:conclusion}

In the paper a unified approach to the adaptive estimation
of the univariate time series parameters have been presented
and specified for two model-selection type methods and one
aggregation method.
The approach has been applied to Gaussian, volatility,
Poisson, exponential and Bernoulli models.
A universal
procedure for the choice of critical values has been developed.
The influence of global
parameters such as the test level on the critical values has been
investigated.
Theoretical properties of the procedures have been investigated
in the most unified way possible so far.
It is hardly possible to pick the best method among the considered
ones. With a good choice of critical values all methods considered
demonstrate very reasonable performance on simulated and real-life
data.



==> intro.tex <==
\section*{Introduction}
\label{sec:intro}

Since ARMA~\citep{boxjenkins}, the classical linear model for
stationary time series, a multitude of extensions for the
nonlinear and non-stationary case has been developed.
Models for nonlinear time series can be divided into two groups: those
modelling nonlinearity in the conditional mean, e.g.\ threshold
auto-regressive model~\citep{tong-lim}, and %
those modelling nonlinearity in the variance, e.g.\ conditional
heteroskedastic (CH) models including ARCH \citep{engle_arch} and
GARCH \citep{bollerslev_garch} and their extensions that have been
inspired by the particular behaviour of financial time series
(``stylized facts'') such as volatility clustering, heavy tails,
asymmetry etc.
Generalizations for the non-stationary case include ARIMA
and ARFIMA
as well as
IGARCH~\citep{nelson_igarch} and FIGARCH~\cite{baillie-figarch}
models for (fractionally) integrated time series.
\citet{fan-vcmodels} give an overview on the modern developments in
the area of varying coefficient models originated
by~\citet{hastie-tibshirani-vc}.

However, the question of whether ubiquitous
financial time series are nonstationary, e.g.\ possess a unit root, or
experience structural breaks has been extensively debated
\citep{nelsonplosser}, \citep{perron}.
It has been shown \citep{mikosch_starica_struc_breaks} that
long range memory effects in financial time series may be caused by
structural breaks rather than result from nonstationarity.
Further it has been argued \citep{diebold_long_memory} that
structural breaks can easily
be overlooked with negative impact on the quality of
modelling, estimation and forecasting \citep{hillebrand_neglecting_changes_ar}.
\citet{perron} introduced a model with breaks that are exogenous,
i.e.\ induced by external influence at known times,
\citet{zivotandrews} suggested a sequential method of testing
for endogenous breaks, i.e.\ not known beforehand.
In this paper we also test for endogenous breaks sequentially and
apply locally parametric estimation methods to stationary subsets
of the series.
Methods of this kind have been presented e.g.\ in \cite{fan_gu_semiparam_var}
for adaptive selection of the decay factor used to weight components of
the pseudo-likelihood function,
in \cite{dahlhaus_rao_tvarch} for the formulation of the locally
stationary ARCH(\( \infty \)) processes,
in \cite{cheng_fan_spokoiny_dyna_nonparam_vola}
for locally choosing parameters of a filter.


The mentioned locally parametric methods
are
the local change point (LCP) procedure \citep{mercurio_lcp},
the local model selection (LMS), also
known as the intersection of confidence intervals (ICI)
\citep{katkovnik06:_spatial}, 
and the stagewise aggregation (SA) \citep{belomestny07:ssa}.
Until present the properties of these procedures
were proven for the corresponding particular cases.
In this paper we present a unified approach to
adaptive estimation upon which the three aforementioned
methods are based,
treat theoretical properties of the estimators in a general way
way and give a universal procedure for the choice of parameters
(\emph{critical values}). 

Another focus of the paper is on the generality of the model.
Modelling financial data involves the use of various
distributions. For instance, the volatility model is applied to study
the dynamics of squared returns, transactions on the market can be
looked at as Bernoulli random events, time between transactions is
usually assumed to follow the exponential or Weibull
distribution, and transaction intensity can be described by the
Poisson distribution.  In this paper a rather general model allowing
for an arbitrary distribution from the exponential family is adopted.
Models of this kind, however with accent of generalized linear models,
have been used to study binary, categorical
and count time series~\citep{FokiKedem2003}.

The paper is organized as follows. Section~\ref{sec:setup} is devoted
to the formulation of the problem in the
context of univariate time series
and theoretical introduction.
Section~\ref{sec:description-meth} describes the local parametric
methods. In the Section~\ref{sec:crit-values} the procedure to
obtain \emph{critical values}, essential parameters of the procedures
is given. Section~\ref{sec:theoprop-adaptive} collects theoretical
properties of the procedures, including the main result, the oracle
inequality, stating that the quality of the adaptive estimates provided
by the procedures is comparable
with the quality of the best possible estimate.
Finally, Section~\ref{sec:simulations} demonstrates
the performance of the procedures on simulated and real data belonging
to various distributions.



==> preamble.tex <==
\usepackage{amssymb}
\newcommand{\newmathcommand}[2]{\newcommand{#1}{\ensuremath{#2}}}
\newcommand{\onehalf}{\ensuremath{^1\kern-.25em/\!_2}}
\newcommand{\cc}[1]{\mathcal{#1}}
\newcommand{\E}{\boldsymbol{\mathrm{E}}}
\newcommand{\indicator}[1]{\ensuremath{{\bf 1}\{ #1 \}}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\ac}[1]{#1} 

\newmathcommand{\obs}{Y}
\newmathcommand{\sigmaalgsym}{\mathcal{F}}
\newcommand{\filtration}[1]{\ensuremath{(\sigmaalgsym_{#1})}}
\newmathcommand{\measuresym}{P}
\newmathcommand{\dommeasure}{\measuresym}
\newmathcommand{\distribfamily}{\mathcal{\dommeasure}}
\newcommand{\measure}[1]{\ensuremath{\boldsymbol{\mathrm{\measuresym}}_{#1}}}
\newcommand{\margindistrib}[1]{\ensuremath{\dommeasure_{#1}}}
\newcommand{\jointdistrib}{\measure}
\newmathcommand{\genparam}{\upsilon}
\newmathcommand{\genparamset}{\Upsilon}
\newmathcommand{\genparamest}{\tilde{\genparam}}
\newcommand{\regfun}[1]{\ensuremath{f(#1)}} 
\newcommand{\paramregfun}[2]{\ensuremath{f_{#1}(#2)}} 

\newmathcommand{\param}{\theta}
\newmathcommand{\paramset}{\Theta}
\newmathcommand{\trueparam}{\param^{*}}
\newmathcommand{\canparam}{v} 

\newmathcommand{\logdensity}{\ell}
\newcommand{\likelihood}[2][{}]{\ensuremath{L_{#1}( #2)}}
\newcommand{\lratio}[3][{}]{\likelihood[#1]{#2, #3}}
\newmathcommand{\density}{p}
\newmathcommand{\weakest}{\tilde{\param}} 
\newcommand{\fitlik}[2]{\lratio[#1]{\weakest_{#1}}{#2}}

\newmathcommand{\interval}{I} 
\newmathcommand{\intlength}{N}

\newmathcommand{\kullbsym}{\mathcal{K}} 
\newcommand{\kullb}[3][{}]{\ensuremath{\kullbsym^{#1}(#2, #3 )}} 
\newcommand{\kldivergence}{Kullback -- Leibler divergence}

\newcommand{\flww}[2]{\ensuremath{\fitlik{#1}{\weakest_{#1}}}}
\newcommand{\flwa}[2]{\ensuremath{\fitlik{#1}{\aggest_{#2}}}}
\newcommand{\flaa}[2]{\ensuremath{\intlength_{#1}} \kullb{\aggest_{#1}}{\aggest_{#2}}}

\newmathcommand{\rpower}{r}
\newcommand{\parametricriskbound}[1]{\ensuremath{\mathfrak{r}_{#1}}}
\newcommand{\loss}[2]{\ensuremath{\rho(#1, #2)}}
\newmathcommand{\risk}{\mathcal{R}}
\newcommand{\riskfun}[2]{\ensuremath{\risk( #1, #2 )}}
\newcommand{\parametricrisk}[3][\trueparam]{\risk_{{#2},{#1},{#3}}}
\newcommand{\maxparametricrisk}[2]{\risk_{#1,#2}}
\newmathcommand{\smbparamrisk}{\parametricrisk[\smbparam]{\rpower}{\smbinterval}}

\newcommand{\rup}[2][\rpower]{\ensuremath{\left\vert #2 \right\vert ^ {#1}}}

\newmathcommand{\testlevel}{\alpha}

\newmathcommand{\divergence}{\Delta}
\newmathcommand{\smbsym}{\circ} 
\newmathcommand{\smbparam}{\param^{\smbsym}}
\newmathcommand{\smbinterval}{\interval^{\smbsym}}
\newmathcommand{\smbdivergence}{\divergence^{\smbsym}}

\newmathcommand{\randomvar}{\zeta}

\newmathcommand{\paramvarbound}{\mathfrak{a}}

\newmathcommand{\mscond}{\cc{A}} 
\newcommand{\changepoint}{\ensuremath{\tau}}
\newcommand{\aggest}{\ensuremath{\hat{\param}}}
\newcommand{\up}[1]{^{(#1)}}
\newmathcommand{\testedinterval}{J}
\newmathcommand{\testinginterval}{\mathcal{I}}
\newmathcommand{\leftsym}{\prime}
\newmathcommand{\rightsym}{\prime\prime}
\newmathcommand{\leftinterval}{\testinginterval^{\leftsym}} 
\newmathcommand{\rightinterval}{\testinginterval^{\rightsym}} 
\newcommand{\intnum}{\ensuremath{k}}
\newmathcommand{\maxintnum}{K}
\newcommand{\nlhi}{\ensuremath{\hat \intnum}}
\newcommand{\teststat}{\ensuremath{T}}
\newmathcommand{\mytime}{t}
\newmathcommand{\rightedge}{\mytime^\diamond}
\newcommand{\starttime}{\rightedge}

\newmathcommand{\confset}{\mathcal{E}}

\newmathcommand{\mixcoeff}{\gamma}
\newcommand{\weik}{\ensuremath{\weakest_i\up{k}}}
\newcommand{\aeik}{\ensuremath{\aggest_i\up{k}}}
\newcommand{\aeikmo}{\ensuremath{\aggest_i\up{k-1}}}

\newcommand{\winwidth}{\ensuremath{a}}
\newcommand{\bandwidthmultiplier}{\ensuremath{d}}
\newcommand{\bandwidth}{\ensuremath{h}}
\newcommand{\weight}{\ensuremath{w}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\Wk}{\ensuremath{W\up{k}}}
\newcommand{\WK}{\ensuremath{W^{(\maxintnum)}}}
\newcommand{\critval}{\ensuremath{\mathfrak{z}}}
\newcommand{\assign}{\ensuremath{\leftarrow}}
\newcommand{\Kag}{\ensuremath{K_\mathrm{ag}}}
\newmathcommand{\barKag}{\bar K_\mathrm{ag}}

\newmathcommand{\B}{\mathbb{B}}

\newmathcommand{\oracleindex}{k^{\smbsym}}
\newmathcommand{\mamoment}{\nu} 

\newmathcommand{\intlenratiolbound}{\intlenratioubound_{0}}
\newmathcommand{\intlenratioubound}{\mathfrak{u}}
\newmathcommand{\varintlenratioubound}{c_{\intlenratioubound}}

\newcommand{\maxcritvalafter}[1]{\bar{\critval}_{#1}}


\newmathcommand{\numrep}{M}
\newmathcommand{\stepheight}{h}
\newmathcommand{\stepdistance}{d}
\newmathcommand{\contrast}{D}
\newmathcommand{\paramlow}{\underline{\param}}
\newmathcommand{\paramhi}{\overline{\param}}
\newmathcommand{\dettime}{\mathfrak{\mytime}}
\newmathcommand{\jumpfraction}{\delta}


\newcommand{\mynote}[1]{}

\newmathcommand{\stockprice}{S}
\newmathcommand{\sqlogret}{Y}
\newmathcommand{\horizon}{h}
\newmathcommand{\inno}{\varepsilon}


